BanFakeNews: A Dataset for Detecting Fake News in Bangla

Observing the damages that can be done by the rapid propagation of fake news in various sectors like politics and finance, automatic identification of fake news using linguistic analysis has drawn the attention of the research community. However, such methods are largely being developed for English where low resource languages remain out of the focus. But the risks spawned by fake and manipulative news are not confined by languages. In this work, we propose an annotated dataset of ~50K news that can be used for building automated fake news detection systems for a low resource language like Bangla. Additionally, we provide an analysis of the dataset and develop a benchmark system with state of the art NLP techniques to identify Bangla fake news. To create this system, we explore traditional linguistic features and neural network based methods. We expect this dataset will be a valuable resource for building technologies to prevent the spreading of fake news and contribute in research with low resource languages.

==> sections/RelatedWork_dataset_.tex <==
\cite{perez-rosas-etal-2018-automatic} collected a dataset of 240 legitimate news from six different domains (sports, business, entertainment, politics, technology, and education). The news was collected from different mainstream news websites in the US. To generate fake versions of the legitimate news items, they used the crowdsourcing via Amazon Mechanical Turk (AMT). They instructed workers to reproduce both a fake headline and the corresponding news body within the same topic and length as the legitimate news. They use a linear SVM classifier with different linguistic features such as N-grams \cite{Scholkopf:2001:LKS:559923}, Punctuations, LIWC \cite{pennebaker2015development} and conduct their evaluations using five-fold cross-validation, with accuracy, precision, recall, and F1-score as performance metrics. Their results show that when using all the features on the two datasets they achieve the best accuracies, with 0.74 and 0.76 respectively. When a  dataset of out of domain set is tested on a model trained on Fake News Dataset the accuracy drops to 0.52. They have also shown that the performance of humans on fake news detection is less than their model. However, their dataset is comparatively small.

The Liar Dataset \cite{wang2017liar} includes 12.8K human-labeled short statements from POLITIFACT.COM's API, and each statement is evaluated by a POLITIFACT.COM editor for its truthfulness. They have used 6 classes ( pants-fire, false, barely-true, half-true, mostly-true, True) for classification of their dataset. They have also included a rich set of meta-data for each speaker of statements such as party affiliations, current job, home state, and credit history. For Automatic Fake News Detection, they have used Surface level linguistic realization and besides they have used a hybrid Convolutional Neural Network to integrate meta-data with text.
Their best performance on fake news detection is 27.4\% on the basis of Accuracy. 

\cite{rashkin-etal-2017-truth} sampled standard trusted news articles from the English Gigaword corpus and crawled articles from seven different unreliable news sites of differing types. 
Trusted News is collected from Gigaword News. 
Satire is collected from The Onion, The Borowitz Report and Clickhole. 
Hoax is collected from American News and DC Gazette. 
Propaganda is collected from The Natural News and Activist Report. 
These news sites are US-based. In total, they have collected  74476 news.
They have taken the main body of the news for their datasets.
To characterize differences between news types, They have applied various lexical resources to trusted and fake news articles. After tokenizing the text with NLTK they compute per-document count for each lexicon and report averages per article of each type. Later on, They trained a Max-Entropy classifier with L2 regularization on n-gram tf-idf feature vectors (up to trigrams). The model achieves F1 scores of 65\% on the out-of-domain test set.

\cite{rubin-etal-2016-fake} collected and analyzed a dataset of 360 news articles from US and Canadian national newspapers. They have collected legitimate and satire articles from 4 different domains (civics, science, business, and ``soft'' news) and with 3 distinct topics within each of the 4 domains.\\
Civics: Gun Violence, Election, Immigrations.\\
Science: Environment, Health, Other Science Topics.\\
Business: Tech, Finance, Corporate Announcements.\\
Soft News: Celebrity, Sports, Local News.\\ 
Each satirical was matched to a legitimate news article that was published in the same country, and as closely related in subject matter as possible. They propose and test a set of 5 satirical news features: Absurdity, Humor, Grammar, Negative Affect, and Punctuation.\\
\textbf{Absurdity}:  The Absurdity Feature (Abs) was defined by the unexpected introduction of new named entities (people, places, locations) within the final sentence of satirical news.\\
\textbf{Humor}: They assigned the binary value (humor=1) when the relatedness between the first and last article sentences was the minimum with respect to the remaining sentences.\\
\textbf{Grammar}: They counted the presence of parts of speech terms including adjectives, adverbs, pronouns, conjunctions, and prepositions, and assigned each normalized value as the element in a feature array representing grammar properties.\\
\textbf{Negative Affect and Punctuation}: Values were assigned based on the presence of negative affect terms and punctuation (periods, comma, colon, semi-colon, question marks, exclamation, quotes).\\  
They tried Support Vector Machine to classify satire and legitimate news using the above 5 features. The F-score(87\%) was maximized in the case when Grammar, Punctuation and Absurdity features were used.

\cite{potthast-etal-2018-stylometric} use a corpus that consisted of three types of news. Mainstream, Right-wing, Left-wing. They have collected in total 1627 news, out of them 826 are mainstream, 256 are left-wing, and 545 are right-wing. And all of them are published on  7 workdays close to the US presidential elections 2016. Four BuzzFeed journalists worked on the manual fact-checks of the news articles. Mainstream news is collected from ABC News, CNN, Politico. Left-wing news is collected from Addicting Info, Occupy Democrats, The Other 98\%. And Right-wing news is collected from Eagle Rising, Freedom Daily, Right Wing News. Each data contains the following items:
Author: Author of the news article\\
Hyperlinks: Links that were included on that news\\
mainText: The contents of the news article\\
Orientation: Political orientation of the news article\\
Paragraph: Extents of one paragraph in the article\\
Portal: The news portal that linked to this news article on their Facebook page.\\
Quote: Extents of a quotation in the article.\\ Quotes that were included in that news
Title: Title of the news article\\
URI: Original URI of the news article\\
Veracity: (Mostly true, Mixture of true and False, Mostly False, No factual content)\\
They have experimented with four baseline models: a topic-based bag of words model, a model using only the domain-specific news style features. and naive baselines. In the style features they have taken N-grams of POS, characters, Stop Words, Ratios of quoted words and external links, Readability scores into account.


\cite{karadzhov-etal-2017-fully} propose a fully automated fack checking system using external links. The system starts with a claim to verify. First, they convert the claim into a query, then search against a search engine in order to get a list of potentially relevant documents. Then, they take both the snippets and the most relevant sentences in the full text of these Web documents, and they compare them to the claim. The features they used are the dense representations of the claim of the snippets and related sentences from the Web pages, which they train for the task using Long Short-Term Memory networks (LSTMs). They also use the final hidden layer of the neural network as a task-specific embedding of the claim, together with the Web evidence. They feed all these representations as features, together with pairwise similarities, into Neural Network and Support Vector Machine (SVM) classifier using an RBF kernel to classify the claim as True or False. They have used a dataset consisted of 761 claims from snopes.com, which span various domains including politics, local news, and fun facts. Each of the claims is labeled as factually true (34\%) or as a false rumor (66\%). 



\cite{karimi-tang-2019-learning} propose a Hierarchical Discourse-level Structure framework for Fake news detection. HDSF learns and constructs a discourse-level structure for fake/real news articles in an automated and data-driven manner. They have uses five available fake news datasets in this study. They have shown that their proposed model outperforms different baselines including N-grams (\cite{Scholkopf:2001:LKS:559923}), LIWC (\cite{pennebaker2015development}), RST(\cite{Rubin:2015:TDR:3150779.3150783}), BiGRNN-CNN(\cite{ren-zhang-2016-deceptive}), LSTM. 
 



\cite{bourgonje2017clickbait} used the dataset from the Fake NewsChallenge (FNC1). Their idea is to check whether a headline is related to the rest of the article or not. To check the relation between a headline and article they have used stance detection. They have also used the credibility or reputation scores of news outlets to make it more functional. Fake NewsChallenge (FNC1) Dataset was annotated for four classes: Unrelated, Agree, Disagree, Discuss. In total there are 49972 news in their collection. They have used linguistic features to detect relation between headline and article. Their system's accuracy is 89.59\%. 


==> sections/relatedWork.tex <==
Few previous studies produced datasets of which some are publicly available. FNC-1 dataset\footnote{\url{www.github.com/FakeNewsChallenge/fnc-1}} consists of headline and body text of news articles, created for fake news challenge. The goal was to encourage and invent new algorithms for stance detection. But this dataset is designed only to help the process of finding stance from a news article. There are some large datasets available such as LIAR \cite{wang2017liar} which is collected using Politifact.com's API is a fine-grained six-class-labeled textual dataset where the labels are pants-fire, false, barely true, half-true, mostly true, and true. They used 10,269 data for training and the size of validation and testing sets are 1284 and 1283, respectively. Getting real about Fake News, a Kaggle dataset\footnote{\url{www.kaggle.com/mrisdal/fake-news}} contains 12,999 posts scraped from 244 websites tagged as "bullshit" by the BS detector, is an initial step to interpret and recognize fake news. Some datasets are collected from different popular social network websites. BuzzFeedNews\footnote{\url{www.github.com/BuzzFeedNews/2016-10-facebook-fact-check}} is a repository with news published close to 2016 US election on Facebook page from nine different news agencies over a week where all the news are fact-checked and labeled as mostly true, a mixture of true and false, and mostly false. Similar social media based dataset is CREDBANK which is crowdsourced from Twitter, including almost 60 million tweets \cite{mitra2015credbank}. Higgs is another twitter dataset which contains four-directional network statistics including social network statistics, retweet network statistics, reply network statistics, and mention network statistics are extracted from the Twitter \cite{de2013anatomy}. This dataset was first used to study the anatomy of a scientific rumor, a kind of misinformation. Despite being an important issue, we have found no such datasets in the Bangla language for detection of fake news. The approaches for detecting fake news, satirical news, rumors, hoaxes depend on various datasets designed accordingly. In our work, we structured the dataset in a way so that it can be useful for multiple lines of research.
